Fundamental Limits of Multiple Sequence Reconstruction from Substrings

The problem of reconstructing a sequence from the set of its length-$k$ substrings has received considerable attention due to its various applications in genomics. We study an uncoded version of this problem where multiple random sources are to be simultaneously reconstructed from the union of their $k$-mer sets. We consider an asymptotic regime where $m = n^\alpha$ i.i.d. source sequences of length $n$ are to be reconstructed from the set of their substrings of length $k=\beta \log n$, and seek to characterize the $(\alpha,\beta)$ pairs for which reconstruction is information-theoretically feasible. We show that, as $n \to \infty$, the source sequences can be reconstructed if $\beta > \max(2\alpha+1,\alpha+2)$ and cannot be reconstructed if $\beta < \max( 2\alpha+1, \alpha+ \tfrac32)$, characterizing the feasibility region almost completely. Interestingly, our result shows that there are feasible $(\alpha,\beta)$ pairs where repeats across the source strings abound, and non-trivial reconstruction algorithms are needed to achieve the fundamental limit.

==> archive.tex <==
\section{Error-Free Decoding Region}

Let us imagine a set of $k$-mers from a set of $M$ strings of length $L$, where each $k$-mer is unique. This is a sufficient yet not necessary condition for all of the $M$ strings to be decoded correctly.
%that is, the set of decoded strings $\hat{S}$ is equal to the set of original strings $S$. 
%and requires not only that any $k$-mer in $s_i$ cannot be the same as any $k$-mer in $s_j$ for $i\neq j$ but also that every $k$-mer in $s_i$ alone must be unique. 
Therefore, the probability that our set of strings can be decoded without error is at least the probability that each of the $k$-mers is generated without error. 

Assuming that all strings are generated independently and uniformly (and therefore, any $k$-mer in $s_i$ is independent of any $k$-mer in $s_j$), the probability that two strings have at least one $k$-mer in common is upper-bounded (using the union bound) by 
\begin{align*}
    \binom{M(L-k+1)}{2} 4^{-k}&\leq M^2L^24^{-k}\\
    &=2^{ 2\log M + 2\log L - 2k }.
\end{align*}

Additionally, we need to consider the case where a single string contains a repeat $k$-mer.
%while this doesn't imply an error has occurred, an error occurring for strings that don't share $k$-mers with each other implies a string has a repeat $k$-mer. 
In this case, not all of the $k$-mers are independent due to their overlapping design. However, even overlapping $k$-mers have a probability of $4^{-k}$ of being the same. Let $k_1$ and $k_2$ be two $k$-mers in the same string and let $t>0$ be the amount that the end of $k_1$ overlaps with the beginning of $k_2$. We can break up the $k$-mers into sub-intervals that are independent. In order for the first $t$ symbols of $k_2$ to be the same as the first $t$ symbols of $k_1$, we need the first and last $t$ symbols of $k_1$ to be the same, which happens with probability $4^{-t}$. Next, we need the last $k-t$ symbols of $k_2$ to be equal to the last $k-t$ symbols of $k_1$, which has a probability of $4^{-(k-t)}$. Therefore,
\begin{align*}
    \text{Pr}(k_1=k_2|t) = 4^{-t}4^{-(k-t)}=4^{-k}.
\end{align*}
So the probability that there is a string that has a repeat $k$-mer is upper-bounded by
\begin{align*}
    ML^24^{-k}=2^{\log M + 2\log L - 2k}.
\end{align*}
%If two $k$-mers from the same string share an overlap of $t$, meaning one $k$-mer $k_1$ begins at position $i$ and the other $k_2$ begins at position $i+(k-t)$, then
%\begin{align*}
%    \text{Pr}(k_1=k_2|t) = 4^{t-k}.
%\end{align*}
%Therefore, the probability there is a repeat $k$-mer in one string is upper-bounded by
\begin{comment}
\begin{align*}
    (L-k+1) (2\sum_{t=1}^{k-1} 4^{t-k} + (L-2k+1)4^{-k} )\\
    =(L-k+1)((L-2k+1)4^{-k}+\frac{1}{3}(2-4^{3/2-k}))\\
    \leq L^24^{-k}+\frac{2}{3}L-\frac{1}{3}L4^{3/2-k}\\
    \leq L^24^{-k}+L-\frac{1}{4}L^{3/2-k}\\
    =L^24^{-k}-L4^{1/2-k}+L\\
    =L4^{-k}(L-2)+L\\
    \leq L^24^{-k}+L
\end{align*}

and so the probability that there is a string with a repeat $k$-mer is upper-bounded by 
\begin{align*}
    ML^24^{-k}+ML
\end{align*}
\end{comment}
\begin{comment}
To force the probability to go to 0 as $M\rightarrow\infty$, the exponent must be negative: 
\begin{align*}
    2\log M+2\log L-2k&<0\\
    \log M+\log L - k&<0\\
    \log(ML)&<k.
\end{align*}
\end{comment}



\section{Giant Component Region}

\section{No Error-Free Decoding Region}

While it is difficult to tell what conditions exactly lead to an error in the solution set, we can characterize when an error will not occur. 

\begin{lemma}
    If there is more than one possible solution set, at least one of the following must be true:
    \begin{enumerate}
        \item There is some $k$-mer index $a$ such that $s_i(a)=s_j(a)$ for two strings $s_i$, $s_j$.
        \item There exist strings $s_i$, $s_j$, $s_l$ (possible that $j=l$) and $k$-mer indices $a$ and $b$ such that the first $k$-mer of $s_i$, $s_i(1)$, is equal to $s_j(a)$, or the last $k$-mer of $s_i$, $s_i(n)$, is equal to $s_l(b)$.
        \item There exist three unique strings $s_i$, $s_j$, $s_l$ and $k$-mer indices $a$, $b$, $c$ such that $s_i(a)=s_j(b)=s_l(c)$.
        \item One of the strings has a repeat $k$-mer. 
        %\item Define \textit{branching points} as $k$-mers that two or more strings have in common and as the first and last $k$-mers of each string. Define \textit{branching paths} as the substrings of $k$-mers including and between each pair of branching points, where the length of a branching path is the number of $k$-mers it contains. Then given a correct decoding of one string $\hat{s}=s_i$ for some $i$ that has branching points, the sum of the lengths of a subset of its branching paths is equal to the sum of the lengths of the branching paths of at least one other string that shares its branching points.
        \item ?
    \end{enumerate}
    
\end{lemma}
\begin{proof}

    %Let us assume that conditions (1)-(4) are all false. With this in mind, we claim that the weight of every edge in the graph---that is, the number of strings containing a given $(k+1)$-mer---is implied by the graph. 
    %We show this by assuming that the first $k$-mer of each string is distinct; if they aren't, the last $k$-mers must be distinct, and we have the same analysis but in reverse. \klcomment{we can actually have some strings w/ overlapping first k-mer, as long as their last k-mers are distinct.}
    %Each string contains $n$ distinct $k$-mers, meaning that a node isn't visited more than once by the same string; therefore, any feasible decoding must include $n$ distinct nodes in each string. 
        %Noting that every non-endpoint node on an Eulerian path must have the same out-degree and in-degree (including edge weights), 
    %We start at $\hat{s}_i(1)$ for all $i$ in a cluster and greedily label each edge with its weight, which is 1 until the first overlap. Since the in-degree of the first overlap node is 2 and no three strings overlap in the same position, the out-degree must be 2, which is represented either by two separate edges each with weight 1 or by one edge with weight 2. 
    %This process continues until either $\hat{s}_1$ or $\hat{s}_2$ has length $n$ nodes; if the $n$th node of one overlaps with a node in the other, then all subsequent outgoing edges have weight 1. 
    %This process continues until all of the strings have length $n$ nodes; if the $n$th node of one string overlaps with a node in another, then all subsequent outgoing edges have weight 1. 

    %Due to condition (1), if a decoding path begins with $s_i(1)$ and then crosses over via an overlap to $s_j$, then the overlap node $s_i(a)$ must be equal to $s_j(a+\Delta)$ for some nonzero $\Delta$. Similarly, since this path must then cross over again to string $s_l$, if the path continues until $s_l(n)$, then if the overlap node between $s_j$ and $s_l$ is at $s_j(b)$, then $s_j(b)$ must be equal to $s_l(b-\Delta)$. This ensures the total path length is $a+b-(a+\Delta)+n-(b-\Delta)=n$.

    \textbf{Probability of event (1)}: 
    \begin{align*}
        \text{Pr}(\exists i,j,a:s_i(a)=s_j(a)) \leq M^2L4^{-k}
    \end{align*}

    \textbf{Probability of event (2)}:
    \begin{align*}
        \text{Pr}(\exists i,j,l,a,b:s_i(1)=s_j(a)\cup s_i(n)=s_l(b)) \leq 2M^2L^24^{-2k}
    \end{align*}

    \textbf{Probability of event (3)}:
    \begin{align*}
        \text{Pr}(\exists i,j,l,a,b,c:s_i(a)=s_j(b)=s_l(c))\leq M^3L^34^{-2k}
    \end{align*}

    \textbf{Probability of event (4)}:
    \begin{align*}
        \text{Pr}(\exists i,a,b:s_i(a)=s_i(b))\leq ML^24^{-k}
    \end{align*}

    If conditions (2)-(4) are not true and a cluster of strings contains an incorrect decoding, then every possible incorrect decoding of the cluster can be described by a path of strings whose substrings are included in a decoding. 
    %For instance, if $s_1$ and $s_2$ make up a cluster and $s_1(a)=s_2(a)$, then a possible incorrect decoding can be described as $s_1\rightarrow s_2$, $s_2\rightarrow s_1$. Define a \textit{junction} as a point where a transition happens, 
\end{proof}

\begin{comment}
\begin{lemma}\label{lm:almost-ind}
    If $k>log(mn)^{3/2}$, the edges in a ``triad'' of strings (i.e., a connected cluster in $H(\mathcal{X})$ that contains three nodes) are approximately independent of each other; that is, the probability of a triad with three edges is dominated by the term $m^3n^62^{-3k}$, which is an upper bound on the probability of a triad in an Erdős-Renyi graph with edge probability $n^22^{-k}$.
\end{lemma}

\textit{Proof:} Denote the event that strings $u$ and $v$ have an edge between them as $u-v$. For any three strings $x_i$, $x_j$, $x_l$, 
\begin{align*}
    \text{Pr}(x_i-x_j,x_j-x_l,x_i-x_l)\leq \underbrace{n^32^{-2k}}_{(a)} + \underbrace{n^62^{-3k}}_{(b)}.
\end{align*}
In the above equation, $(a)$ represents the ``dependent'' terms. Note that given $x_i(a)=x_j(b)$ and $x_j(b)=x_l(c)$ for three indices $a$, $b$, $c$, then $x_i(a)=x_l(c)$ with probability 1 by transitivity. Therefore, $(a)$ represents the event that there is a $k$-mer that appears in all three strings. Meanwhile, $(b)$ represents the ``independent'' terms, or the terms that are equal to the product of the marginal edge probabilities. The probability that there are any three strings that form such a triad is therefore upper-bounded by
\begin{align*}
    \text{Pr}(\text{triad})\leq \underbrace{m^3n^32^{-2k}}_{(c)}+\underbrace{m^3n^62^{-3k}}_{(d)}.
\end{align*}

We wish for term $(c)$ to approach zero for a larger region of $k$, $m$, and $n$ than for term $(d)$. Setting the exponent of $(c)$ to be negative, we find the condition $k>\log(mn)^{3/2}$, whereas for term $(d)$ we need $k>\log (m^{3/2}n^2)$. Therefore, $(d)$ approaches zero only if $(c)$ does as well. \qedwhite

Using Lemma \ref{lm:almost-ind}, if $k>\log(mn)^{3/2}$, the edges in a triad can be treated as independent
\begin{align*}
    \binom{m}{3}n^42^{-2k}\leq 2^{3\log m+4\log n-2k}.
\end{align*}
This probability goes to zero if and only if 
\begin{align*}
    k>\log (m^{3/2}n^2)
\end{align*}
which, since $\alpha>2$, is less than $\log (m^2n)$.

\vspace{1cm}

\textbf{Probability of event (1)}: 
    \begin{align*}
        \text{Pr}(\exists i,j,a:s_i(a)=s_j(a)) \leq M^2L4^{-k}
    \end{align*}

    \textbf{Probability of event (2)}:
    \begin{align*}
        \text{Pr}(\exists i,j,l,a,b:s_i(1)=s_j(a)\cup s_i(n)=s_l(b)) \leq 2M^2L^24^{-2k}
    \end{align*}

    \textbf{Probability of event (3)}:
    \begin{align*}
        \text{Pr}(\exists i,j,l,a,b,c:s_i(a)=s_j(b)=s_l(c))\leq M^3L^34^{-2k}
    \end{align*}

    \textbf{Probability of event (4)}:
    \begin{align*}
        \text{Pr}(\exists i,a,b:s_i(a)=s_i(b))\leq ML^24^{-k}
    \end{align*}

\end{comment}

\begin{comment}
\subsection{Achievability}

We aim to find $\beta$ such that $\Pr(\E_k)\to 0$ for $k=1,2,3$, thus capturing a range of $(\alpha,\beta)$ parameters where multiple sets $\X$ could have generated $\Y$. 

\subsubsection{Special case: $\alpha > 2$}

$\E_1$ is the event that one string contains a repeat $k$-mer. Note from the previous section that $\Pr(\E_1)\leq mn^22^{-k}=2^{\log m+2\log n-k}$, so $$\Pr(\E_1)\to 0\text{ if }\beta>\alpha+2.$$

Similarly, the probability of $\E_2$ is upper-bounded by $m^2n2^{-k}=2^{2\log m+\log n-k}$, so $$\Pr(\E_2)\to 0 \text{ if }\beta>2\alpha+1.$$

We can define $\E_3$ as the union of two events, $\E_{3,A}$ and $\E_{3,B}$, where
\begin{itemize}
    \item $\E_{3,A}=\{ \exists i,j,l,a,b,c,d:\x_i(a)=\x_j(b),\x_i(c)=\x_l(d) \}$
    \item $\E_{3,B}=\{ \exists i,j,a,b,c,d:\x_i(a)=\x_j(b),\x_i(c)=\x_j(d) \}$
\end{itemize}

$\E_{3,A}$ represents the event that there is a connected cluster of size three or greater in $G_S(\mathcal{X})$. Since edges in $G_S$ are pairwise independent, \klcomment{are they?} the probability that there exist two edges between three nodes is upper-bounded by 
\begin{align*}
    3m^3n^42^{-2k}&=3\cdot 2^{3\log m + 4\log n -2k}\\
    &=3\cdot 2^{(3\alpha + 4)\log n-2k}.
\end{align*}
This bound goes to zero if and only if $\beta > \frac{3}{2}\alpha+2$. 

%Note that the probability that there is a repeat $k$-mer in one string goes to zero when $\beta > \alpha + 2$, so the probability of this event goes to zero if the probability that there are two edges between three nodes as well. Therefore, as long as $\beta > \frac{3}{2}\alpha + 2$, connected components in $H$ have size at most 2 with probability going to 1. 

Further, $\E_{3,B}$ is the event that one string shares multiple $k$-mers with any other string. If two $k$-mers are shared between two strings, they are either consecutive in both strings or independent of each other. Consecutive shared $k$-mers can be treated as a single shared $(k+1)$-mer, so we seek to find $\beta$ such that the probability of two shared independent $k$-mers goes to zero. An upper bound on this probability is given by 
\begin{align*}
    m^2n^42^{-2k}=2^{2\log m + 4\log n - 2k},
\end{align*}
which goes to zero if and only if $\beta > \alpha+2$. 

Therefore, $$\text{Pr}(\E_3)\to 0\text{ if }\beta>\frac{3}{2}\alpha+2.$$

The three lower bounds on $\beta$ that enforce $\Pr(\E)\to 0$ are $\beta_1=\alpha+2$, $\beta_2=2\alpha+1$, and $\beta_3=\frac{3}{2}\alpha+2$. Any $\beta>\beta_3$ is also greater than $\beta_1$, and since $\alpha>2$, $\beta_2>\beta_3$. Therefore, for $\beta>2\alpha+1$, $\Pr(\E)\to 0$.  

\subsubsection{$\frac{3}{2}<\alpha<2$} According to the lower bounds on $\beta$ computed in the previous section, when $\alpha<2$ it is not clear that the event $\E_2$ dominates $\E$. Here, meeting the condition for the probability of $\{\exists i,j,a:x_i(a)=x_j(a)\}$ to go to zero does not imply that the probability of a cluster of size three or greater in $G_S(\X)$ will also go to zero. 

In order to find when a cluster of size three implies $\E$, we can again define $\E_3$ as the union of several events:
\begin{itemize}
    \item $\E_{3,A}=\{\exists i,j,l,a,b:\x_i(1)=\x_j(a),\x_i(n-k+1)=\x_l(b)\text{ for }j=l\text{ or }j\neq l\}$
    \item $\E_{3,B}=\{\exists i,j,a,b,c,d:\x_i(a)=\x_j(b),\x_i(c)=\x_j(d)\}$
    \item $\E_{3,C}=\{\exists i,j,l,a,b,c,d,e,f:\x_i(a)=\x_j(b),\x_i(c)=\x_l(d),\x_j(e)=\x_l(f)\}$
    %\item $\E_{3,D}=\{ \exists i,j,a,b,c,d:\x_i(a)=\x_j(b),\x_i(c)=\x_j(d) \}$
    \item $\E_{3,D}=\{\exists h,i,j,l,a,b,c,d,e,f:\x_h(a)=\x_i(b),\x_i(c)=\x_j(d),\x_j(e)=\x_l(f)\}$
    \item $\E_{3,E}=\{ \exists i,j,a,b,c,d:\x_i(a)=\x_j(b),\x_i(c)=\x_j(d) \}$
\end{itemize}

$\E_{3,A}$ is the event that the first and last $k$-mer of one string appear in at least one other string. An upper bound on its probability is
$$m^2n^22^{-2k}+m^3n^22^{-2k}$$
which goes to zero if and only if $\beta > \frac{3}{2}\alpha+1. $

$\E_{3,B}$ is the event that there are two $k$-mers in common between a pair of strings, which we found in the previous section has probability approaching zero if and only if $\beta>\alpha+2$.

$\E_{3,C}$ is the event that there is a fully-connected cluster of size three in $G_S(\X)$. Note that these edges are not mutually independent; if there are edges between $\x_i(a)$ and $\x_j(b)$ and between $\x_j(b)$ and $\x_l(c)$ for some $\x_i$, $\x_j$, $\x_l$ and $k$-mer indices $a$, $b$, $c$, then there is an edge between $\x_i(a)$ and $\x_l(c)$ with probability 1. Therefore, the probability of $\E_{3,C}$ can further be divided into this case of dependent edges and cases where all edges are independent:
$$\Pr(\E_{3,C})\leq m^3n^32^{-2k}+m^3n^62^{-3k}$$.
This upper bound goes to zero if and only if $\beta>\max(\frac{3}{2}\alpha+\frac{3}{2},\alpha+2)$. If $\alpha>1$, then this lower bound is $\beta>\frac{3}{2}\alpha+\frac{3}{2}$.

$\E_{3,D}$ is the event that there is a cluster in $G_S(\X)$ of size four or greater.

With events $\E_{3,A}$ through $\E_{3,D}$ having probability approaching zero, 

%$\E_2$: overlap in same position --- $2\alpha+1$

%$\E_{3,A}$: size 3 or greater --- $\frac{3}{2}\alpha+2$

%$\E_{3,B}$: 2 $k$-mers shared with other string --- $\alpha+2$

%$\E_{3,A'}$: size 4 or greater --- $\frac{4}{3}\alpha+2$

%$\E_{3,B'}$: 3 $k$-mers shared between 2 or 3 strings --- $\alpha+2$



% \begin{align*}
%     m^2n^22^{-(k+1)}&\leq m^2n^22^{-k}\\
%     &=2^{2\log m + 2\log n -k}.
% \end{align*}
% This bound goes to zero if and only if $\beta>2\alpha+2$. 

%In summary, $\beta>\frac{3}{2}\alpha+2$ is a regime where the largest cluster size is 2 with high probability, there are no non-consecutive $k$-mers shared between two strings with high probability, and no string contains a repeat $k$-mer with high probability. Therefore, the only error case is that when there is a pair of strings $x_i$, $x_j$ and a $k$-mer index $a$ such that $x_i(a)=x_j(a)$, which happens with probability
%\begin{align*}
%     \text{Pr}(\exists i,j,a:x_i(a)=x_j(a))&\leq m^2n2^{-k}\\
%     &=2^{2\log m + \log n - k}.
%\end{align*}
%This bound goes to zero if and only if $\beta>2\alpha+1$. Since $\alpha>2$, $2\alpha+1>\frac{3}{2}\alpha+2$, so if $\beta>2\alpha+1$, correct recovery of $\mathcal{X}$ is possible with probability going to 1. 

%$\beta>\alpha+2$: no repeat $k$-mer in one string

%$\beta>2\alpha+2$: no $k$-mer shared between two strings

%When $\alpha<2$, however, the region where there are no overlaps in the same position does not guarantee a maximum cluster size of 2, as $2\alpha+1$ is less than $\frac{3}{2}\alpha+2$. We examine the case where $1<\alpha<2$, so that having no shared $k$-mers in the same position on a pair of strings implies that each string shares at most one $k$-mer with any other string and that there are no repeat $k$-mers in any string. 
\end{comment}

Define $Z_{i,j}=\sum_{a=1}^{n-k+1}\mathbbm{1}_{\{\x_i(a)=\x_j(a)\}}$, and let $V=\sum_{i=1}^m\sum_{j> i}\mathbbm{1}_{\{Z_{i,j}>0\}}$. Note that $\E_1 = \{V>0\}$.

By the Paley-Zygmund inequality, the probability that there is at least one pair of strings that shares a $k$-mer in the same position is lower bounded as
$$
\text{Pr}(V>0)\geq \frac{\mathbb{E}[V]^2}{\mathbb{E}[V^2]}.
$$
It is straightforward to calculate $\mathbb{E}[Z_{i,j}]=(n-k+1)2^{-k}$, 
%\iscomment{this is not exact right? there are $n-k+1$ $k$-mers. }
and therefore $\mathbb{E}[V]=m(m-1)(n-k+1)2^{-k}$. Additionally,
\begin{align*}
    \mathbb{E}[V^2]&=\mathbb{E}\left[ \sum_{i=1}^m\sum_{j>i}\mathbbm{1}_{\{Z_{i,j}>0\}}\sum_{s=1}^m\sum_{t> s}\mathbbm{1}_{\{Z_{s,t}>0\}} \right]\\
    &=\mathbb{E}\left[\sum_{i=1}^m\sum_{j> i} \mathbbm{1}_{\{Z_{i,j}>0\}}\mathbbm{1}_{\{Z_{i,j}>0\}} \right]\\
    &\quad + 2\mathbb{E}\left[\sum_{i=1}^m\sum_{j>i} \mathbbm{1}_{\{Z_{i,j}>0\}}\sum_{s\neq i}\sum_{\substack{t> s}} \mathbbm{1}_{\{Z_{s,t}>0\}} \right]\\
    &=\mathbb{E}\left[ \sum_{i=1}^m\sum_{j>i}\mathbbm{1}_{\{Z_{i,j}>0\}} \right] \\
    &\quad + 2\mathbb{E}\left[\sum_{i=1}^m\sum_{j> i} \mathbbm{1}_{\{Z_{i,j}>0\}}\sum_{s\neq i}\sum_{\substack{t> s}} \mathbbm{1}_{\{Z_{s,t}>0\}} \right]\\
    &=m(m-1)(n-k+1)2^{-k}\\
    &\quad+2(m(m-1)(n-k+1)2^{-k})^2.
\end{align*}
%\iscomment{I don't understand the steps above. Where do the 2 and the 4 come from? Can you add some clarification steps?}
%\klcomment{my bad --- wasn't thinking about equivalence between $Z_{i,j}$ and $Z_{j,i}$}
% \iscomment{I'm confused about the second line in the equation above. What does it mean to have a sum over $s=i$ or over $t=j$?}
Therefore, with $\gamma=m(m-1)(n-k+1)2^{-k}$ for brevity,
\begin{align*}
    \text{Pr}(V>0)&\geq \frac{\gamma^2}{\gamma+2\gamma^2}\\
    &=\frac{1}{\frac{1}{\gamma}+2}
    %&\geq \frac{(m(m-1)(n-k+1)2^{-k})^2}{m^2n2^{-k}+2(m^2n2^{-k})^2}\\
\end{align*}
which approaches $\frac{1}{2}$ asymptotically as long as $\beta<2\alpha+1$.
